Multi-task closed-loop inverse kinematics stability through semidefinite programming

Today's complex robotic designs comprise in some cases a large number of degrees of freedom, enabling for multi-objective task resolution (e.g., humanoid robots or aerial manipulators). This paper tackles the stability problem of a hierarchical losed-loop inverse kinematics algorithm for such highly redundant robots. We present a method to guarantee system stability by performing an online tuning of the closedloop control gains. We define a semi-definite programming problem (SDP) with these gains as decision variables and a discrete-time Lyapunov stability condition as a linear matrix inequality, constraining the SDP optimization problem and guaranteeing the stability of the prioritized tasks. To the best of authors' knowledge, this work represents the first mathematical development of an SDP formulation that introduces stability conditions for a multi-objective closed-loop inverse kinematic problem for highly redundant robots. The validity of the proposed approach is demonstrated through simulation case studies, including didactic examples and a Matlab toolbox for the benefit of the community.

==> sections/simulation_bu.tex <==

\section{Validation}
\label{sec:validation}

% \sout{Gain tuning} 
\comb{Task stabilization through the optimization procedure presented in this work is of use when dealing with highly redundant robots that must perform several tasks.
In these cases, the analytical analysis to choose the right gains, hence to guarantee stability, becomes unfeasible.
% \sout{(\ie when the number of variables to consider is high)}
% \comb{In this kind of robots, the analytical analysis becomes too complex. 
When the number of tasks and required DOFs are not high (\eg 2 tasks and 3 DOFs), this method is also of use as it eases the search of the gains that will render all tasks stable, without the need for simplifications as in other existing methods (\eg it allows to consider different gains for each task dimension).}

% \sout{However, u}

\comb{The effectiveness of the mathematical developments proposed in this work can be better shown with robots with a low number of DOFs.} 
Hence, without loss of generality and similar to~\cite{antonelli_stability_2009}, we first present a numerical experiment with a 3-link planar manipulator performing two tasks.
Then, we include the simulations using the commercial UR5\footnote{\scriptsize\url{https://www.universal-robots.com/products/ur5-robot/}} robot arm performing with the on-line task gain tuning approach.
These examples suffice to validate
% \sout{the optimization solution adopted and the role of every LMI presented in the previous section.}
\comb{that:
\begin{enumerate}
	\item[a)] In all simulations the stability condition in~\eqref{eq:stability_condition} holds. 
	This can be checked by looking at the highest eigenvalue of the sum in \eqref{eq:lyapunov_finalcondition}, which has to be negative as sign for stability.
	\item[b)] Variations on $\tilde{\beta}$ truly affect the convergence speed. For higher values of $\tilde{\beta}$ the tasks should converge faster.
	\item[c)] Joint velocity bounds $\overline{\dbfq}, \underline{\dbfq}$ are respected and the system still manages to converge by relaxing $\beta$.
	\item[d)] The method can handle different values of $\Delta t$ without affecting the system stability.
\end{enumerate}}

% \sout{For this purpose, we take} 
\comb{We have performed the simulations by taking }advantage of \texttt{Matlab} and the toolbox presented in \cite{corke_robotics_2017} to simulate a robot manipulator.
Moreover, we use the already existing SDP solver \texttt{Sedumi}~\cite{sturm_using_1999}.
% Moreover, we added the capability of solving the SDP problem with both the SDPA solver \cite{yamashita_latest_2012} and Sedumi~\cite{sturm_using_1999}.
All code related with this paper is made publicly available for the benefit of the community%
\footnote{\scriptsize\url{https://gitlab.iri.upc.edu/jmarti/SDP_HierarchicalTaskStability}}.

\subsection{3-link planar manipulator}

For this case study, the mission consists of accomplishing two tasks.
A first task is set to drive the end-effector to a desired position and a second one to reach a desired end-effector orientation.
The current values for both tasks are specified conveniently with $\bfsigma_1 \inR^2$ and $\sigma_2 \inR$ for position and orientation, respectively, with their initial values set to ${\bfsigma_1(0) = [0.5, 0]^\top\text{m}}$ and ${\sigma_2(0) = -1.134\,\text{rad}}$.
In the following experiments, we have set ${\bfsigma^\ast_{1} = [0.76, 0.18]^\top \text{m}}$ and ${\sigma^\ast_{2} = -1.22\,\text{rad}}$ as desired task values.
The serial manipulator has 3 links of lengths ${L = [0.5, 0.3, 0.2]\,\text{m}}$.
\comb{In all the problems we have considered a regularization value of $\delta=2\cdot 10^{-5}$.}

% \sout{In order to validate the proposed approach we present here two main groups of experiments based on varying either the $\beta$ parameter in~\eqref{eq:stability_condition_mod_2} or the sampling time $\Delta t$.
% In both groups we have departed from the same SDP with the following paramterization of $\bfF_2$ and $\bfF_3$: we have considered a bound for the joint velocity of $\overline{\dbfq} = -\underline{\dbfq} = [3.0, 3.0, 3.0]^\top \text{rad/s}$ and desired gains of $\tilde{\bflambda} = [1, 1, 10] \text{s}^{-1}$.
% Then, in the first groups we have set a fixed constant $\Delta t=0.01\text{s}$ with varying $\beta$.
% On the contrary, in the latter group we have considered a fixed \sout{$\beta = 0.05$} \comb{0.5} with varying $\Delta t$.}

\begin{figure}[t]
	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_stability.pdf}
	\vspace{-2em}
	\caption{Maximum eigenvalue of the sum in \eqref{eq:lyapunov_finalcondition} for the 3DOF planar manipulator case. 
	Constant gains (solid blue), $\tilde{\beta} = 2$ (dashed red), $\tilde{\beta} = 8$ (dotted yellow). The reported values must negative to guarantee stability.}
	\label{fig:3dof_stability}
	\vspace{-1em}
\end{figure}

\comb{We have done several experiments to validate the items a)-d) stated above.
Although the system stability (a) has been confirmed in all simulations, for the sake of conciseness, it is only reported here the stability figure of the experiments where we want to show the efectiveness of $\tilde{\beta}$.
In those, we have set $\Delta t = 0.01\text{s}$ and $\overline{\dbfq} = -\underline{\dbfq} = [3.0, 3.0, 3.0]^\top \text{rad/s}$ and ran several simulations to compare our method with both $\tilde{\beta} = 2$ and $\tilde{\beta} = 8$ against the tasks deployment with $\bflambda = [1,1,10]^\top$ as fixed gains.
% \sout{In this simulation, we validate our approach by checking that~\eqref{eq:stability_condition} holds at every time instant, \ie that both tasks are stable during their deployment.
% We do so by checking the maximum eigenvalue of the sum in \eqref{eq:lyapunov_finalcondition}, which has to be negative for stability.
% This eigenvalue is plot \figref{fig:3dof_stability}, where we are comparing an experiment done by assuming constant gains with values $\bflambda = [1,1,10]^\top$ during the whole experiment (blue continuous line in \figref{fig:3dof_stability}) to the case of using the proposed SDP approach for different $\tilde{\beta}$ values.}
The corresponding results are shown in \figref{fig:3dof_stability}, where the stability of the CLIK method is not guaranteed when using constant $\bflambda$ gains the (notice the positive maximum eigenvalue indicated by the solid blue line).
Although in this case this has no effect on the tracking error for the primary task, shown in \figref{fig:3dof_eepos}, it does for the second one, shown in \figref{fig:3dof_eeori}, where using constant gains the error cannot be completely driven towards zero.
For the sake of readability, all plots for this robot type are time-cropped to $5s$.
Besides, we can see in \figref{fig:3dof_eepos} and \figref{fig:3dof_eeori} that the convergence speed of both tasks is increased if $\tilde{\beta}$ has higher values.}

\begin{figure}[t]
\vspace{-1em}
  \begin{tabular}{lr}
      \rotatebox{90}{\hspace{-2.5em}a) Position error.} & \hspace{-1.5em}
\begin{subfigure}{.5\textwidth}
	\includegraphics[width=0.8\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_eepos.pdf}
	\captionlistentry{}
	\label{fig:3dof_eepos}
\end{subfigure} \vspace{-0.5em} \\ \vspace{-0.5em}
      \rotatebox{90}{\hspace{-3em}b) Orientation error.} & \hspace{-1.5em}
\begin{subfigure}{.5\textwidth}
	\includegraphics[width=0.8\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_eeori.pdf}
	\captionlistentry{}
	\label{fig:3dof_eeori}
\end{subfigure}
\end{tabular}
\vspace{-0.5em}
\caption{End-effector error norms considering different values of $\tilde{\beta}$ for the 3DOF planar manipulator case. Constant gains (solid blue), $\tilde{\beta} = 2$ (dashed red), $\tilde{\beta} = 8$ (dotted yellow).}
\label{fig:fig}
\vspace{-0.5em}
\end{figure}

% \sout{Notice how the maximum eigenvalue is smaller than $0$ only using our gain tuning approach.}

% \begin{figure}[t!]
%     \vspace{-1em}
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_eepos.pdf}
% 	\vspace{-1em}
% 	\caption{End-effector position error norm considering different values of $\tilde{\beta}$ for the 3DOF planar manipulator case. Constant gains (solid blue), $\tilde{\beta} = 2$ (dashed red), $\tilde{\beta} = 8$ (dotted yellow).}
% 	\label{fig:3dof_eepos}
% \end{figure}
% \begin{figure}[t!]
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_eeori.pdf}
% 	\vspace{-1em}
% 	\caption{End-effector orientation error norm considering different values of $\tilde{\beta}$ for the 3DOF planar manipulator case. Constant gains (solid blue), $\tilde{\beta} = 2$ (dashed red), $\tilde{\beta} = 8$ (dotted yellow).}
% 	\label{fig:3dof_eeori}
% \end{figure}

% \begin{figure}
% \begin{subfigure}{.5\textwidth}
%   \centering
%     \vspace{-1em}
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_eepos.pdf}
% 	\vspace{-1em}
% 	% \begin{turn}{90}
% 	\caption*{\rotatebox{90}{ a) Position error norm.}}
% 	% \end{turn}
% 	\label{fig:3dof_eepos}
% \end{subfigure}

% \begin{subfigure}{.5\textwidth}
%   \centering
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_eeori.pdf}
% 	\vspace{-1em}
% 	\caption*{b) Orientation error norm.}
% 	\label{fig:3dof_eeori}
% \end{subfigure}
% \caption{End-effector error norms considering different values of $\tilde{\beta}$ for the 3DOF planar manipulator case. Constant gains (solid blue), $\tilde{\beta} = 2$ (dashed red), $\tilde{\beta} = 8$ (dotted yellow).}
% \label{fig:fig}
% \end{figure}

% \comb{\sout{By definition in \eqref{eq:stability_condition_mod_2}, higher values of $\beta$ translate to faster error convergence for all tasks.
% This effect is shown in \figref{fig:3dof_eepos} and \figref{fig:3dof_eeori} for the primary and secondary tasks, respectively.}}
\begin{figure}[t!]
    \vspace{-1em}
	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_Kori.pdf}
	\vspace{-1em}
	\caption{Gain associated to the orientation task considering different values of $\tilde{\beta}$ for the 3DOF planar manipulator case, with constant gains (solid blue), $\tilde{\beta} = 2$ (dashed red) and $\tilde{\beta} = 8$ (dotted yellow).}
	\label{fig:3dof_Kori}
	\vspace{-2em}
\end{figure}
\begin{figure}[t!]
  % \smallskip
  % \vspace{-1em}
	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_jointvel.pdf}
	\vspace{-1em}
	\caption{Limited joint velocities when $\tilde{\beta} =8$ and $\overline{\dbfq}=-\underline{\dbfq} = [2.0, 2.0, 2.0]^\top \text{rad/s}$ for the 3DOF planar manipulator case. Joint 1 (solid blue), joint 2 (dashed red), joint 3 (dotted yellow).}
	\label{fig:3dof_jointvel}
	\vspace{-0.5em}
\end{figure}

\begin{figure}[t!]
    \vspace{-1em}
	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_beta.pdf}
	\vspace{-1em}
	\caption{$\beta$ value for different values of $\overline{\dbfq}$ and $\underline{\dbfq}$. Fixed value of $\tilde{\beta} = 8$.  $\overline{\dbfq}=-\underline{\dbfq}= [3.0, 3.0, 3.0]^\top \text{rad/s}$ (solid blue), $\overline{\dbfq}=-\underline{\dbfq} = [2.0, 2.0, 2.0]^\top \text{rad/s}$ (dashed red).}
	\label{fig:3dof_beta}
	\vspace{-2em}
\end{figure}
\begin{figure}[t!]
    \vspace{-1em}
	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/3dof_dt_eeori.pdf}
	\vspace{-1em}
	\caption{End-effector orientation norm error considering different $\Delta t$ for the 3DOF planar manipulator case. Fixed $\tilde{\beta}=8$. $\Delta t = 0.1$s (solid blue), $\Delta t = 0.05$s (dashed red), $\Delta t = 0.01$s (dotted yellow), $\Delta t = 0.005$s (dashed magenta).}
	\label{fig:3dof_dt_eeori}
	\vspace{-1.5em}
\end{figure}

% \sout{As it has been noted before,} 
\comb{In this experiment}
the manipulator is driven towards a singularity and therefore, towards a situation where the null-space of the first task becomes smaller\comb{, hence the joint velocities devoted to fulfill the low priority task become smaller.}
When operating in a close-loop manner, this vanishing joint velocity can be tackled by increasing the gains\comb{,
a benefit of imposing~\eqref{eq:stability_condition_mod} within our SDP approach}.
% This is done in the SDP approach as a consequence of imposing~\eqref{eq:stability_condition_mod}.
This effect is shown in~\figref{fig:3dof_Kori}, where the orientation task gain is increased as the configuration approaches the singularity.
% This gain increase can lead to undesired high joint velocities, and to mitigate this we have added a joint velocity constraint, acting during the first part of the experiment, for the second link, as shown in~\figref{fig:3dof_jointvel}.

\comb{As previously noted, imposing faster error dynamics by increasing $\tilde{\beta}$ results in increasing the joint velocities.
This fact might violate the joint velocity constraint ($\bf F_2$) if the $\beta$ was not properly relaxed ($\bf F_3$).
This case is shown in \figref{fig:3dof_jointvel}, where the limits for the joints' velocities are respected while the $\beta$ value is moved away from its desired $\tilde{\beta}$ (\figref{fig:3dof_beta}), in order to keep the joints' velocity limits while guaranteeing the system stability.
Notice that \figref{fig:3dof_beta} shows how $\beta$ is modified differently depending on the imposed joint velocity limits.}

% The sampling time $\Delta t$ is also of importance when considering the stability of the CLIK algorithm.
% In the following figures, we illustrate how the proposed method successfully incorporates the sampling time into the stability analysis.
% As one could suspect looking at~\eqref{eq:stability_condition_mod_2}, for a fixed value of $\beta$, the gains that make this LMI hold are different depending on the value of $\Delta t$.
% More precisely, the gains will be different for those $\Delta t$ values that make the quadratic term $\bfA^\top\bfA\Delta t$ not negligible.
% An important remark is that for a sufficiently small $\Delta t$, the quadratic term vanishes and~\eqref{eq:stability_condition_mod_2} becomes the stability condition of the continuous-time CLIK algorithm.
% This fact is shown in~\figref{fig:3dof_dt_Kori}, where the optimal gains of the orientation task converge to a specific solution as $\Delta t$ decreases.
% In~\figref{fig:3dof_dt_eeori}, we show that, even though $\Delta t$ is different, the orientation error dynamics are similar.
% Furthermore, the positioning error has no remarkable difference within the different sampling times considered and its plot has been avoided for sake of space.

\comb{The effect of the sampling time in the system performance is depicted in \figref{fig:3dof_dt_eeori}.
Even though the same value for $\tilde{\beta}$ has been kept across all different $\Delta t$, low values on $\Delta t$ results in slower error convergence speed.
An important remark is that for a sufficiently small $\Delta t$, the quadratic term vanishes and~\eqref{eq:stability_condition_mod_2} becomes the stability condition of the continuous-time CLIK algorithm.
This fact is shown in~\figref{fig:3dof_dt_eeori}, where the error trajectory seems to converge to a specific solution as $\Delta t$ decreases.}

\como{\bf AS: I am here}

\subsection{UR5 arm manipulator}
In this example, we perform a simulation with the commercial robotic arm UR5 ($6$ DOFs) to reproduce a hand-writing action done by a human arm.
With this aim, we set a primary task to follow a desired position path with the robot's end effector, whose error is described by $\tilde{\bfsigma}_1\inR^3$.
Besides, we impose the wrist to be close to the writing surface as a secondary task, \ie we impose the $y$ coordinate of the 4th joint to have a specific value ($\tilde{\sigma}_2\inR$).
% \sout{In this experiment, the manipulator is driven towards a configuration where the two tasks are close to be dependant.
% This behavior is produced using the first task (higher priority).}
\comb{In this experiment, the manipulator is driven towards a configuration where the two tasks are close to be dependant, \ie where the rank of the augmented Jacobian is smaller than the sum of ranks of the respective Jacobians.}
In such a situation, the secondary task gain has to be increased to guarantee overall stability.
% Hence, the gain of the second task has to be tuned to guarantee the system stability.
The parameters for this case study are \mbox{$\bfq_0 = [135, 0, -90, 0, 90, 0]^\top \text{deg}$},
\mbox{$\bfsigma_{1}^\ast = [-0.5,-0.4,0.6]^\top \text{m}$}
and \mbox{$\sigma_{2}^\ast  = -0.3 \text{m}$}.
% \begin{equation} \label{eq1}
% \begin{split}
% \bfq_0 & = [135, 0, -90, 0, 90, 0]^\top \text{ deg} \,, \\
% \tilde{\bfsigma_{1}} & = [-0.5,-0.4,0.6]^\top \text{ m} \,, \\
% \tilde{\bfsigma_{2}} & = -0.3 \text{ m} \,. \\
% \end{split}
% \end{equation}
% Besides, we have fixed all values of \sout{$\bflambda_1 = [2,2]^\top$} \comb{$\bflambda_1 = [2,2,2]^\top$} so the stability is reached through the proper tuning of $\lambda_2$.
\comb{Besides, we have considered a $\tilde{\beta} = 8$ and also limited all joint velocities to $6 \text{rad/s}$.
As in the experiments with the 3DOF manipulator, 
our method has been compared against fixed constant gains $\bflambda = [2,2,2,1]^\top$.
Again, the pattern for the maximum eigenvalues shown for the previous robot is here repeated: 
while the SDP-based method is able to guarantee the stability, the maximum eigenvalue for the fixed gains is positive, leading to a tracking error in the secondary task (see \figref{fig:ur5_wr_error}).
All variations on $\tilde{\beta}$, joint velocity bounds and sampling time have been evaulated for the UR5 robot model, resulting in similar behaviors as the ones observed for the 3 DOF robot.
So, the corresponding plots have been omitted for the sake of brevity.}

\begin{figure}[t]
	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/ur5_eewr.pdf}
	% \vspace{-1em}
	\caption{Second task error norm for the UR5 arm manipulator case. Constant gains (solid blue), $\tilde{\beta} = 8$ (dashed red). $\Delta t = 0.01$s.}
	\label{fig:ur5_wr_error}
	\vspace{-1.5em}
\end{figure}
% \begin{figure}[t!]
%     \vspace{-1em}
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/ur5_stability.pdf}
% 	\vspace{-1em}
% 	\caption{Maximum eigenvalue of the sum in \eqref{eq:lyapunov_finalcondition} for the UR5 arm manipulator case. It must be negative for stability. Constant  \sout{$\lambda_2 = 10$} \comb{$\lambda_2 = 1$} (solid blue), \sout{$\beta = 1.5$} \comb{$\beta = 0.5$} (dashed red). $\Delta t = 0.01$s.}
% 	\label{fig:ur5_stability}
% \end{figure}
% \begin{figure}[t!]
%     % \vspace{-1em}
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/ur5_Kwr.pdf}
% 	\vspace{-1em}
% 	\caption{Second task gain, $\lambda_2$, for the UR5 arm manipulator case. Constant  \sout{$\lambda_2 = 10$} \comb{$\lambda_2 = 1$} (solid blue), \sout{$\beta = 1.5$} \comb{$\beta = 0.5$} (dashed red). $\Delta t = 0.01$s.}
% 	\label{fig:ur5_wr_gain}
% \end{figure}
% \begin{figure}[t!]
% 	\includegraphics[width=0.9\columnwidth, angle=0, trim={30 20 80 20},clip]{figures/ur5_sv.pdf}
% 	\vspace{-1em}
% 	\caption{Minimum singular value to show dependency between tasks. Constant  \sout{$\lambda_2 = 10$} \comb{$\lambda_2 = 1$} (solid blue),\sout{$\beta = 1.5$} \comb{$\beta = 0.5$} (dashed red). $\Delta t = 0.01$s.}
% 	\label{fig:ur5_sv}
% \end{figure}

% The effect of using the SDP gain tuning approach is shown in~\figref{fig:ur5_wr_error} and \figref{fig:ur5_stability}.
% Setting a fixed gain for the second task (\ie $\lambda_2$) does not allow for error convergence towards zero, since the maximum eigenvalue is greater than zero (solid blue line in~\figref{fig:ur5_wr_error} and \figref{fig:ur5_stability}, respectively).
% Instead, using the SDP to tune the gain online, the stability is guaranteed and the error is nullified (dashed red in~\figref{fig:ur5_wr_error} and \figref{fig:ur5_stability}, respectively).
% The values of $\lambda_2$ for this same experiment are shown in~\figref{fig:ur5_wr_gain}.
% Besides, the dependency between tasks is illustrated in \figref{fig:ur5_sv}, showing the minimum singular value of the matrix $\bfJ_2\overline{\bfN}_{1}\bfJ_2^\dagger$ from \eqref{eq:error_velocity_error}.
% In this figure, values close to $0$ indicate that the tasks are close to be dependant.
% Notice how when this dependency appears, the respective gain is correspondingly increased guaranteeing the system stability.
